Studying the anonymity trilemma with a discrete-event mix network simulator

In this work, we present a discrete event mix network simulator, which allows analysing how anonymity, latency, and bandwidth overhead are affected by various scenarios of deployment and design choices. These design choices include network topology, mixing technique, volume of traffic, latency requirements, packet size or use of cover traffic. To the best of our knowledge, this is the first such simulator as work on it began in 2017 to analyze the Loopix mix network, and the code of our simulator is available under an open-source license. To demonstrate the capabilities of our simulator, we perform an empirical analysis of the impact of core design choices on anonymity, scalability and latency in Elixxir, HOPR and Nym, currently deployed mix network infrastructures that make a variety of different choices in their design.

==> sections/framework.tex <==
\section{Framework}\label{sec:framework}

The better understanding of the dependencies between the privacy guarantees of the mix networks and their technical properties can help in the future deployment of such systems. Hence, we aim to study the relation of the network parameters with
privacy loss and the overall performance of the mix network. For this purpose, we closely monitor its operation using various metrics collected from different network components. In this section, we first define the \emph{network parameters} which we consider in our measurements. Next, we detail the metrics used in our analysis to quantify security or performance, and investigate how different system parameters influence those metrics.

\subsection{Network parameters}\label{sec:parameters}

\paragraph{Network topology} 
The first decision when designing an anonymity network is whether to use a \emph{p2p} or a \emph{client-server} architecture. In p2p topology participating peers act as both end users and relay nodes that route the data packets of others, while client-server architecture has a clear distinction of roles between the end users, who send and receive anonymous data packets, and the relays or mix nodes that provide the service to those users. 
In the anonymous communication literature systems like~\cite{} adopt for client-server architecture, while~\cite{} opted for a p2p topology~\cite{}. 
Similarly to the Chaumian mixnet, both Elixxir and Nym are designed as the client-server architectures, while HOPR, on the other hand, is a p2p network. 

% The network topology has a direct impact on scalability, which is a key property of any anonymous communication network as \emph{anonymity loves company}~\cite{}. 

\paragraph{Latency}


\paragraph{Cover traffic}

\input{sections/metrics.tex}

==> sections/metrics.tex <==
\subsection{Anonymity metrics}\label{sec:metrics}

\paragraph{\textbf{Entropy}}
% 
A common measure of anonymity is the \emph{anonymity set}, which reflects the size of the set of other packets with which a given message can be confused by the attacker. 
However, an adversary observing a mix for a period of time may assign different probabilities for each outgoing packet being in terms of being linkable to a given observed incoming packet. 
Different probabilities of observation being given to different members of the anonymity set in lieu of past observations reveal a lot of information to the attacker that is not captured by a simple metric like the anonymity set. Therefore in order to measure the anonymity we use the concept of \emph{Shannon entropy}, introduced in~\cite{}, which allows us to reason about the information contained in this kind of probability distribution. By using entropy as a measure of anonymity, we gain a measure of how indistinguishable the packets shuffled by the mix network are among each other and hence how uncertain the adversary is in determining which of the outgoing packets is their target packet.  

% In order to measure entropy, we simulate an attacker who observes packets traversing the mixnet. 
% The adversary observes the target sender injecting a packet $p_X$ into the mix network. The adversary can observe the entire network, and the intermediate links between nodes. To each packet leaving a mix network, the adversary assigns a probability $p_i$ of it being the earlier observed packet $p_X$.  


\paragraph{\textbf{Third-party unlinkability}}

Let $A$ and $B$ denote events that the sender of the target packet was $\mathsf{S_A}$ or $\mathsf{S_B}$ respectively. As $\epsilon$ we denote the measure of information leaked by the system and define it as
\begin{align*}
    \epsilon = \log \left( \frac{\Pr(A)}{\Pr(B)} \right)
\end{align*}
In contrast to~\cite{}, we assume that the adversary can observe the the network over multiple rounds, during which $\mathsf{S_A}$ or $\mathsf{S_B}$ are sending packets. Multiple observations increases the adversary’s advantage. From the Law of Large numbers~\cite{}, we know that for large number of repeated experiments the average of the results converges to the expected value of the outcomes. Hence, in order to compute the anonymity leakage of an observed round $R_i$ we compute the value of $\hat{\epsilon}$ for a large number of samples $K$ as follows
\begin{align*}
  \hat{\epsilon} = \frac{1}{K} \sum_{i=1}^K \log \left(\frac{\Pr_i(A)}{\Pr_i(B)}\right)
\end{align*}

This allows us to compute the average case leakage, instead of assuming the worst case leakage as for example in the \emph{differential privacy composition theorem}~\cite{}.
Thus, the overall advantage after $R$ observations can be expressed as $\epsilon_R = R\cdot \hat{\epsilon}$.


==> sections/results.tex <==
\section{Experiments & Results}\label{sec:experiments}

\subsection{Scalability}

\emph{Anonymity loves company}~\cite{}, hence scalability is one of the key properties of a mix network. At first sight, P2P architectures may look like a great choice for a privacy network given the general scalability properties of such networks. However, as our analysis shows P2P networks although scale scale easily, provide very poor anonymity despite an increasing number of users. This is an expected result as 

